Inverse Nonlinear Scattering by a Metric

We study the inverse problem of determining a time-dependent globally hyperbolic Lorentzian metric from the scattering operator for semilinear wave equations.

==> reconstruction.tex <==
\section{Detection of Singularities}\label{sec_detection}
Let $\ups_j = (p_j, w_j) \in L^+_{S_+}M$, for $j=1,2,3$.
Recall in previous version, we constructed receding waves and we introduced the following notations
\[
\gamma_j= \gamma_{p_j, w_j},
\quad \Sigma_j=\Sigma({p_j, w_j, s_0}),
\quad K_j = K({p_j, w_j, s_0}), \quad \Lambda_j = \Lambda({p_j, w_j, s_0}).
\]
For each $(p_j, w_j)$, we construct conormal distributions
$\Ups_j \in {\teal {I}^{\mu +1} (\Sigma_j)}$ as receding waves.
Let $v_j$ be the solution to $\sq_g v_j = 0$ with $\lR_-[v_j] = \Ups_j$, for $j = 1, 2, 3$.
Note that $v_j \in {\teal {I}^{\mu - \frac{1}{2}}(\Lambda_j)}$ are conormal distributions away from the point $\{x_j\}$, before the first cut point, for $j = 1,2,3$.
To define a three-to-one scattering relation determined by the radiation field, we introduce the following singularities detection condition as in \cite{Kurylev2018}.

\begin{df}\label{def_D}
    We say a vector $\ups_0 \in L^+\Omgout$ satisfies the \textbf{condition (D)}  with light-like vectors $(\ups_1, \ups_2, \ups_3) \in (L^+\Omgin)^3$ and $\hat{\ka} >0$,
    if
     \begin{itemize}
        \item[(a)] $\ups_0, \ups_1, \ups_2, \ups_3$ are corresponding to distinct null geodesics;
        \item[(b)] for any $0< \ka_0 < \hat{\ka}$ and $j = 1, 2, 3$,  there exists $\Ups_j \in I^{\mu}(\Sigma(p_j,w_j,\ka_0))$ satisfying the support condition (\ref{assump_fj2}), where $(p_j, w_j) = \ups_j$;
    \end{itemize}
    such that the corresponding covector of
    $\ups_0$ is contained in  $\wfset(\partial_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3} \mcn(\Ups) |_{\epsilon_1 = \epsilon_2 = \epsilon_3=0})$, where $\Ups = \sum_{j=1}^{3} \epsilon_j \Ups_j$.
\end{df}
By this singularity detection condition, we can tell if singularities produced by the interaction of three distorted plane waves emanating from $(\vec{p}, \vec{w})$ at the past null infinity can be detected at the covector $(p_0, w_0^\flat)$ at the future infinity,
where $(\vec{p}, \vec{w})$ are given by $\ups_1, \ups_2, \ups_3 \in L^+_{S_-}M$ and $(p_0, w_0)$ is given by $\ups_0 \in L^+_{S_+}M$.

We introduce the following lemmas.
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lm}\label{lm_Nk}
    Let $\ups_i \in L^+\Omgin$.
    Suppose $A = \gamma_{\ups_1}(\mathbb{R}_+) \cap \gamma_{\ups_2}(\mathbb{R_+}) \cap J(\ymi, \ypl) =  \{q_1, \ldots, q_m \}$ and there exist $(p_j, w_j) \in \lA(\ups_j)$, for $i=1,2$.
    Let $N_k$ be disjoint small open neighborhoods of each $q_k \in A$.
    Then with $\ka_0 > 0$ sufficiently small, we have
    \[
    K({p_1}, {w_1}, \ka_0) \cap  K(x_2, w_2, \ka_0)\cap J(\ymi, \ypl)  \subseteq \cup_{k=1}^m N_k.
    \]
\end{lm}
\begin{proof}
    %Recall the definition of $K(x_0, w_0, s_0)$ and $\mathcal{W}(x_0, w_0, s_0)$ in Section \ref{subsec_planewaves}.
    In the following, we denote %$\gamma_{{p_i}, w_i}(\mathbb{R_+})$ by $\gamma_{w_i}$,
    $K({p_i}, w_i, \ka_0)$ by $K_i$ and ${W}({p_i}, w_i, \ka_0)$ by ${W}_i$, for $i = 1,2$.
    %for the definition see Section \ref{subsec_planewaves}.
    We notice that if $q' \in K_1 \cap K_2$, then there exist
    $(p_i', {w}_i') \in {W}_i$ satisfying $q' \in \gamma_{{p_1'}, {w}_1'}(\mathbb{R}_+) \cap \gamma_{p_2', {w}_2'}(\mathbb{R}_+)$.
    Therefore, it suffices to show that with small enough $\ka_0$, we have
    \[\gamma_{{p_1'}, w'_1}(\mathbb{R}_+) \cap \gamma_{p_2', w_2'}(\mathbb{R}_+) \cap J(\ymi, \ypl) \subseteq \cup_{k=1}^m N_k,
    \]
    for any $(p_i', w_i') \in {W}_i$, for $i=1,2$.
    This is true according to Lemma \ref{lm_Nk_0} by setting
    \[
    \ups'_i = (\gamma_{p_i', w_i'}(-\ep), \dot{\gamma}_{p_i', w_i'}(-\ep))
    \]
    for $i=1,2$ and some $\ep> 0$,  assuming $\ka_0$ is sufficiently small.
    %    We prove this by contradiction.
    %    Assume this is not true.
    %    Then we can find two sequences $w_{i,j}, i=1,2$ such that
    %    $w_{i,j} \rightarrow w_i$ in $\mathcal{W}_i$ as $j \rightarrow \infty$, with $p_j \in \gamma_{{p_1}, w_{1, j}}(\mathbb{R}_+) \cap \gamma_{x_2, w_{1, j}}(\mathbb{R}_+)\cap J({\ymi, \ypl})$ and $p_j \in M \setminus (\cup_{k=1}^m N_k)$.
    %    Since $J({\ymi, \ypl})$ is compact, it has a subsequence converging to some point $p$ and we abuse the notation to denote this subsequence still by $\{ p_j\}$.
    %    Since $M \setminus (\cup_{k=1}^m N_k)$ is closed, we have $p \in M \setminus (\cup_{k=1}^m N_k)$.
    %    For each $j$, since $p_j$ is the intersection point,
    %    we can write $q_j = \gamma_{\ups'_{i,j}}(t_{i,j})$ for $i = 1,2$.
    %    %For convenience, we denote $\gamma_{\ups_0}$ by $\gamma_0$ and $\gamma_{\ups'_{j,k}}$
    %    Note that $p_j  = \gamma_{\ups_j}(t_{i,j}) \rightarrow p$.
    %    By Lemma \ref{lm_convg}, there exists $t_i$ such that $t_{i,j} \rightarrow t_i$ for $i=1,2$.
    %    On the other hand, since the exponential map are continuous, we have $ \gamma_{{p_i}, w_{i,j}}(t_{i,j}) %\rightarrow \gamma_{\ups'_{j, k}}(t_j)
    %    \rightarrow \gamma_{{p_i}, w_{i}}(t_i)$ for $i=1,2$, as $j \rightarrow +\infty$.
    %    It follows that $ p = \gamma_{{p_i}, w_i}(t_i) \in A$, which contradicts with the fact that
    %    $p \in M \setminus (\cup_{k=1}^m N_k)$.
\end{proof}

\begin{lm}
    Let $(\vec{p}, \vec{w})_{j=1}^3 \subseteq L^+_{\Uin} M \cap T^+_{\Uin} M$
    be causally independent as in (\ref{assump_xj}).
    If $q' \in J({\pmi, \ppl})$ such that $(q', \zj) \in \Lambda(x_j, w_j, s_0)$, for $j=1,2,3$,
    then with sufficiently small $\ka_0 > 0$
    %Suppose for any $s_0 \in (0, \hat{s})$, there exists $p \in J({\ymi, \ypl})$ such that $(p, \zj) \in \Lambda(x_j, w_j, s_0)$, for $j=1,2,3$.
    we have
    \begin{itemize}
        \item[(1)] $\zi + \zj \neq 0$, for $ 1\leq i < j \leq 3$,
        %$\Lambda_j + \Lambda_k$ is away from the zero section, for $ 1\leq j < k \leq 3$,
        \item[(2)] $\zeta^{1} + \zeta^{2} + \zeta^{3} \neq 0$.
        %$\Lambda_1 + \Lambda_2 + \Lambda_3$ is away from the zero section.
    \end{itemize}
\end{lm}
\begin{proof}
    We claim that with $\ka_0 > 0$ small enough, we can find $q \in {\cap_{j=1}^{3}\gamma_{{{p_i}, w_i}}(\mathbb{R_+})}$ and $q'$ is in a small neighborhood of $q$.
    Indeed, let $A = {\cap_{j=1}^{3}\gamma_{{{p_i}, w_i}}(\mathbb{R_+})} \cap J({\ymi, \ypl})$.
    By Lemma \ref{lm_finite}, the nonempty set $A$ is finite so we can assume $A = \{q_1, \ldots, q_m \}$.
    Let $N_k$ be disjoint arbitrarily small open neighborhoods of each $q_k \in A$.
    Then Lemma \ref{lm_Nk} implies $q' \in N_k$ for some $k \in \{1, \ldots, m\}$, if $\ka_0$ is sufficiently small.
    %Thus, $(p, \zj) \in \Lambda(x_j, w_j, s_0)$,
    Now suppose $q_k = \gamma_{{{p_i}, w_i}}(\varsm_j)$.
    We notice that $\dot{\gamma}_{{{p_i}, w_i}}(\varsm_j) \in L_{q_k}^+M$, $j = 1,2, 3$, are not multiples of each other,
    which implies
    \[
    c_i \dot{\gamma}_{{p_i}, w_i}(t_i) + c_j \dot{\gamma}_{x_j, w_j}(t_j) \neq 0,
    \quad \text{if }c_i, c_j \neq 0, i,j \in \{1,2,3\}.
    \]
    and by \cite[Lemma 6.21]{feizmohammadi2021inverse} one has
    \[
    c_1 \dot{\gamma}_{{p_1}, {w_1}}(t_1) + c_2 \dot{\gamma}_{p_2, w_2}(t_2) + c_3 \dot{\gamma}_{p_3, w_3}(t_3) \neq 0,
    \quad \text{if }c_1, c_2, c_3 \neq 0.
    \]
    With $\ka_0$ small enough,  the lightlike covector $(q', \zj)$ are sufficiently small perturbations of lightlike covectors
    $(q_k, (c_j \dot{\gamma}_{p_j, w_j}(t_j))^b )$ for some nonzero constant $c_j$.
    Thus, we have the desired result.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
The following lemma is the result of the propagation of singularities, for example, see \cite[Theorem 2.1]{Taylor2017}.
\begin{lm}\label{lm_propagation}
    Let $(p, \eta) \in L^{*,+}_{S_+} M$ and $v$ be the solution to
    \[
    (\sq_g + V) v = f, \quad \lR_-[v]  = 0.
    \]
    %be the solution to
    %\begin{equation*}
    %\begin{aligned}
    %\square_{g}  u &= f, & \  & \mbox{on } M ,\\
    %u &= 0, & \ &\mbox{on } M\setminus J^+(\supp (f)).
    %\end{aligned}
    %\end{equation*}
    Then $(y, \eta) \in \wfset(v)$ only if $(y, \eta) \in \wfset(f)$ or there exists $(q, \zeta)$ such that
    $(q, \zeta) \in \wfset(f)$ and $(p, \eta)$ is contained in the null bicharacteristics starting from $(q, \zeta)$.
\end{lm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%For $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$, we make the following assumptions:
%\begin{equation}\tag{I}\label{assumption_I}
%    \begin{aligned}
%        &\text{${\ups_i}$ and ${\ups_j}$ are not identical, for $ 0 \leq i < j \leq 3$,}\\
%    \end{aligned}
%\end{equation}
%%\begin{enumerate}[\label = \hspace{0.5cm}(\ref{assumption_I})]
%%    \item  \makeatletter\def\@currentlabel{B}\makeatother
%%    \label{assumption_I}
%%\begin{enumerate}[\label = \hspace{0.5cm}(1)]
%%    \item $\gamma_{\ups_i}$ and $\gamma_{\ups_j}$ are not identical, for $ 0 \leq i < j \leq 3$,
%%    \item $(\vec{x}, \vec{\xi})_{j=1}^3$ are causally independent as in (\ref{assump_xj2}).
%%\end{enumerate}
%%\end{enumerate}
%{\teal Note that this assumption can be checked using...}

\begin{prop}\label{pp_intersectempty}
    %For $s_0 >0$ sufficiently small,
    Let $\ups_j$ and $(p_j, w_j)$ be defined as above, for $j = 0, \ldots, 3$.
    If \[(\capgammathree) \cap J(\imi, \ipl)= \emptyset,\] then
    %$(y, \eta) \notin \wfset(\mathcal{U}^{(3)})$ and
    $\ups_0$ does not satisfy the condition (D) with $(\ups_1, \ups_2, \ups_3)$ and small $\hat{s} >0$.
\end{prop}
\begin{proof}
    To check the condition (D), recall $v_l \in I^\mu(\Lambda_l), l=1,2,3$ are Lagrangian distributions away from $p_j$ and we consider the term $w_{1,1,1}$, which is the solution to
    \[
    \square_g w_{1,1,1} -  6v_{1}v_{2}v_{3} = 0, \qquad
    \mathcal{R}_-[w_{1,1,1}] = 0.
    \]
    The goal is to show $(p_0, w_0^\flat) \notin \wfset(\lR_+(w_{(1,1,1)}))$.
    {\teal Let $p'_{-2} > p_{-2}$ be a point such that $V \subset I(p'_{-2}, p_{+2})$.
    Note that $\supp(v_1 v_2 v_3) \subset J^+(p'_{-2})$.
    Let $\chi$ be a smooth cutoff function supported in $J(p_{-2}, p_{+2})$ with $\chi = 1$ in $J(p'_{-2},y)$.
    Then $\supp((1-\chi)v_1 v_2 v_3) \cap J^-(y) = \emptyset$.
    By Lemma \ref{lm_propagation}, one has $(y, \eta) \notin \wfset(Q_g((1- \chi)v_1 v_2 v_3))$.
    Thus, it suffices to check if $(y, \eta)$ is in $\wfset(Q_g(\chi v_1 v_2 v_3))$ and we focus on the set $J(p_{-2}, p_{+2})$.}

    Recall we assume $(\capgammathree) \cap J(\ymi, \ypl)= \emptyset$.
    First, we consider the case where locally there are exactly two null geodesics
    intersecting at one point.
    Suppose $\gamma_i$ and $\gamma_j$ intersect at a point $p$ with $p \notin \gamma_k$,  where $\{i,j,k\} = \{1,2,3\}$.
    With $s_0$ small enough we can suppose $p \notin K_k$.
    Since $v_k$ is smooth near $p$, the wave front set of $v_i v_j v_k$ at $p$ is in the span of $\Lambda_i$ and $\Lambda_j$, by the H\"{o}rmander-Sato Lemma, for example see \cite[Theorem 1.3.6]{Duistermaat2010}.
    Next, we consider the case that none of three geodesics intersect with each other.
    Then we have $\wfset(v_i v_j v_k) \subseteq \cup_{j=1}^3 \Lambda_j$.
    %With $s_0$ small enough we can assume $\cap_{j=1}^3 K_j = \emptyset$.
    %Note that we could have cut points before $p$ along $\gamma_i$ or $\gamma_j$.
    %In general $v_l \in \Ical^\mu(\Lambda_l)$ are Lagrangian distributions associated with the Lagrangian submanifold $\Lambda_l$.
    %may not be a conormal distribution supported in $K_l$, $l = 1,2,3$.
    %We consider the wave front set of a model term $Q_g(v_i v_j v_k)$ using
    In both cases,
    we have
    \[
    \wfset(v_1v_2v_3) \in (\cup_{j=1}^3\Lambda_j) \cup (\cup_{j\neq k \in \{1,2,3\}} \Lambda_j + \Lambda_k),
    \]
    where $\Lambda_j + \Lambda_k \coloneqq \{(q, \zeta^1 + \zeta^2): (q, \zeta^1) \in \Lambda_j, \ (q, \zeta^2) \in \Lambda_k \}$.
    Note that if $(p, \eta)$ is in  $\wfset(\lR(w_{1,1,1}))$, then we must have either $(p, \eta) \in \wfset(v_1v_2v_3)$ or there exists $(q, \zeta) \in \wfset(v_1v_2v_3)$ satisfying $(p, \eta)$ in the null bicharacteristics starting from ${q, \zeta}$ by Lemma \ref{lm_propagation}.

    For the first situation, we must have $(p,\eta)$ contained in $\Lambda_j$ for some $j = 1,2,3$, which is impossible if $s_0$ is small enough.
    %Since $\pi(\Lambda_j)$ tends to $\gamma_{x'_j, \xi'_j}(\mathbb{R}_+)$ as $s_0 \rightarrow 0$, we can always choose $\hat{s}$ small enough such that with $s_0 \in (0, \hat{s})$ one has $y \notin \pi(\Lambda_j)$.
    For the second situation, first we consider if there exists such $(p, \zeta) \in \Lambda_j$ for some $j \in \{1,2,3\}$. % and sufficiently small $s_0$.
    This is impossible, otherwise we have $(y, \eta) \in \Lambda_j$ again.
    Next, we consider if $(q, \zeta) \in \Lambda_i + \Lambda_j$ for some $i,j \in \{1,2,3\}$.
    % and sufficiently small $s_0$.
    If so, then we must have $\zeta = \zi + \zj$ with $(q, \zi) \in \Lambda_i$ and $(q, \zj) \in \Lambda_j$.
    Recall that if a covector $\zeta = \zi + \zj$ is lightlike, then we must have $\zeta$ is propositional to either $\zi$ or $\zj$ by \cite{Kurylev2018}.
    Then $(q, \zeta)$ is contained in  either $\Lambda_i$ or $\Lambda_j$.
    By the analysis above, this is impossible.
    %
    %and the propagation of singularities in Lemma \ref{lm_propagation}.
    %Indeed,
    %Let $(p, \zeta^{(i)}) \in \Lambda_i$ and $(p, \zeta^{(j)}) \in \Lambda_j$.
    %If a covector $\zeta = \zi + \zj$ is lightlike, then we must have $\zeta$ is propositional to either $\zi$ or $\zj$ by \cite{Kurylev2018}.
    %Thus, there are no new singularities produced other than $\cup_{j=1}^3 \Lambda_j$, if we apply $Q_g$ to $v_i v_j v_k$.
    %Next, we consider the case that none of three geodesics intersect with each other.
    %We have $\wfset(v_i v_j v_k) \subset \cup_{j=1}^3 \Lambda_j$ and it follows that
    %$\wfset(Q_g(v_i v_j v_k)) \subset \cup_{j=1}^3 \Lambda_j$.

    Thus, we can conclude that $(p, \eta) \notin \wfset(\lR_+(w_{(1,1,1)}))$ for sufficiently small $s_0$.
    %with the assumption $y \notin \uniongammathree$, if $s_0$ is sufficiently small.
%%%%%%%%%%%%%
%    For the terms in form of $Q_g(\cjv_iv_jv_k)$ or $Q_g(\lge A_1, \diff v_i \rge_g \cjv_j v_k)$, %, or $\lge A_1, \diff \cjv_i \rge_g v_j v_k$,
%    we only need to note that $\wfset(\cjv_i)$ or $\wfset(\lge A_1, \diff v_i\rge)$ is contained in  $\Lambda_i$.
%%%%%%%%%%%%%
    Therefore, one has $(p, \eta) \notin \wfset(\Uthree)$, which implies the condition (D) is not satisfied.
\end{proof}
%Combining Lemma \ref{lm_propagation} and Proposition \ref{pp_intersectempty}, we have the following corollary.
%\begin{corollary}\label{cl_intersectempty}
%%For $s_0 >0$ sufficiently small,
%Let $(y, \eta) \in T^{*,+}V$ such that %$y \in \nxxi$ and
%$y \notin \uniongammathree$.
%If $\capgammathree \cap J(p_{-2}, p_{+2}) = \emptyset$, then
%%$(y, \eta) \notin \wfset(\mathcal{U}^{(3)})$ and
%$(y, \eta)$ does not satisfy the condition (D) with $(\vec{x}, \vec{\xi})_{j=1}^3$ and $\hat{s} >0$ small enough.
%\end{corollary}
%Then we have the following proposition.
%\begin{prop}\label{pp_wfU3}
%    For $s_0 >0$ sufficiently small, let $(y, \eta) \in T^{*,+}V$ such that %$y \in \nxxi$ and
%    $y \notin \uniongammathree$.
%    We have the following statements.
%    \begin{itemize}
    %        \item[(1)] If $\capgammathree = \emptyset$, then
    %        %$(y, \eta) \notin \wfset(\mathcal{U}^{(3)})$ and
    %        $(y, \eta)$ does not satisfy the condition (D) with $(\vec{x}, \vec{\xi})_{j=1}^3$ and $\hat{s} >0$ small enough.
    %        \item[(2)]
    %        Assume $(\capgammathree) \cap \nxxi = \{q\} $ %\subset \mathcal{O}(A_1)$
    %        such that $q = \gamma_{x_j, \xi_j}(t_j)$ with $0 < t_j < \rho(x_j, \xi_j)$, $j=1,2,3$.
    %        %$ \gamma_{x_j, \xi_j}$ intersect regularly at $q$, i.e. if
    %        Suppose $(\dot{\gamma}_{x_j, \xi_j}(t_j))^b$ are linearly independent %at $q$
    %        and $\zeta \in L^{*,+}_qM$ is in their span.
    %        Suppose the assumption (\ref{assumption_Ah}) holds.
    %        %Suppose $q \in  I(p_-,p_+ )$ and the assumption (\ref{assumption_Ah}) hold.
    %        %Assume $ q \in  \mathcal{O}(A_1)$ and the assumption (\ref{assumption_Ah}) hold.
    %        %Suppose $q \in  \mathcal{O}(A_1)$.
    %        If %$ q \in  \mathcal{O}(A_1)$ and
    %        $(y, \eta) \in \mathcal{C}^{\text{reg}}(q, \zeta, t_y)$ for some $t_y>0$, then
    %        $(y, \eta)$ satisfies the condition (D) with $(\vec{x}, \vec{\xi})_{j=1}^3$ and $\hat{s} >0$ small enough.
    %        \item[(3)] Using the source-to-solution map, one can determine if the condition (D) is valid for the given $(y, \eta) \in L^{*,+}V$, $(\vec{x}, \vec{\xi})_{j=1}^3$, and $\hat{s} >0$.
    %        %(? $q \in  \mathcal{O}(A_1)$)
    %    \end{itemize}
%\end{prop}


%
%For convenience, we define $\RLN$ as the set containing $(w_0, w_1, w_2, w_3) \in  L^{+}V$ such that
%$\gamma_{\ups_j}$ are not identical and
%$y \in \nxxi$,
%if we write
%$(y, \eta^\#) = w_0$ and $(\vec{x}, \vec{\xi})_{j=1}^3 = (w_1, w_2, w_3)$.
%This subset of $L^{+}V$ allows us to focus on the nonlinear interaction of waves before caustics.
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lm}\label{lm_xprimej}
%    Suppose $\Gammaset  = \emptyset$ and
%    we write $(y, \eta)  =\ups_0^\#, (\vec{x}, \vec{\xi})_{j=1}^3 = (w_1, w_2, w_3)$.
%    For sufficiently small $s_1 > 0$, if $\ups'_j \in L^+V$, $j = 1, 2, 3$ are in the $s_1$-neighborhood of $\ups_j$, then we must have $\Gammasetprime = \emptyset$.
%\end{lm}
%\begin{proof}
%    %By Lemma \ref{lm_finite}, the set $A = \capgammathree \cap J(p_{-2}, p_{+2})$ is finite and we can assume $A  = \{q_1, q_2, \ldots, q_m\}$.
%    %Consider
%    Note that $\Gammaset$ and $\Gammasetprime$ are contained in $J(p_{-2}, p_{+2})$.
%    It suffices to show that $\Gammasetprime \cap J(p_{-2}, p_{+2}) = \emptyset$, provided $\Gammaset \cap J(p_{-2}, p_{+2}) = \emptyset$ and $s_1$ small enough.
%    Let $A = {\cap_{j=1}^{3}\gamma_{\ups_j}(\mathbb{R_+})} \cap J(p_{-2}, p_{+2})$.
%    By Lemma \ref{lm_finite}, the nonempty set $A$ is finite.
%    When $A = \emptyset$, one can show ${\cap_{j=1}^{3}\gamma_{\ups_j}(\mathbb{R_+})} \cap J(p_{-2}, p_{+2}) = \emptyset$ by Lemma \ref{lm_threeempty}, if $s_1$ is sufficiently small.
%    Otherwise, we assume $A = \{q_1, \ldots, q_m \}$.
%    There exist small open neighborhood $N_k$ of $q_k$ such that $\gamma_{\ups_0} (\mathbb{R_-}) \cap N_k = \emptyset$, $k=1, \ldots, m$.
%    Using Lemma \ref{lm_Nk_0}, we have ${\cap_{j=1}^{3}\gamma_{\ups'_j}(\mathbb{R_+})}\cap J(p_{-2}, p_{+2}) \subset \cup_{k=1}^m N_k$, if $s_1$ is sufficiently small.
%    This implies $\Gammasetprime = \emptyset$.
%    %    We prove by contradiction.
%    %    Assume for arbitrarily small $s_1$, we can find some $\ups'_j = (\xprimej)$ in the $s_1$-neighborhood such that the intersection is not empty.
%    %    More specifically, we can choose a sequence $s_1^k \rightarrow 0$ with $\ups'_{j,k} = (\xprimejk)$ in the $s_1^k$-neighborhood of $(x_j, \xi_j)$, such that there exists $q_k \in \Gammasetprimek$ for each $k \in \mathbb{N}$. %, as $k \rightarrow +\infty$.
%    %    Note that the sequence $\{q_k\}$ is contained in the compact set $J(p_{-2}, p_{+2})$.
%    %    Then it has a subsequence converging to some $q \in J(p_{-2}, p_{+2})$ and we abuse the notation to denote this subsequence still by $\{ q_k\}$.
%    %    For each $k$, since $q_k$ is in the intersection point, we can write $q_k = \gamma_{\ups_{0}}(t_{0,k})$  and $q_k = \gamma_{\ups'_{j,k}}(t_{j,k})$ for $j = 1, 2, 3$.
%    %    %For convenience, we denote $\gamma_{\ups_0}$ by $\gamma_0$ and $\gamma_{\ups'_{j,k}}$
%    %    Note that  one has $q_k =  \gamma_{\ups_{0}}(t_{0,k}) \rightarrow q$
%    %    and $q_k  = \gamma_{\ups_j}(t_{j,k}) \rightarrow q$ for $j = 1, 2, 3$.
%    %    By Lemma \ref{lm_convg}, there exists $t_j$ such that $t_{j,k} \rightarrow t_j$ for $j = 0, 1, 2, 3$.
%    %    On the other hand, since the exponential map are continuous, we have $\gamma_{\ups_{0}}(t_{0,k}) \rightarrow \gamma_{\ups_{0}}(t_0) $ and $ \gamma_{\ups'_{j,k}}(t_{j,k}) %\rightarrow \gamma_{\ups'_{j, k}}(t_j)
%    %    \rightarrow \gamma_{\ups_j}(t_j)$ for $j=1,2,3$, as $k \rightarrow +\infty$.
%    %    It follows that $ q = \gamma_{\ups_{0}}(t_0) = \gamma_{\ups_j}(t_j)$, which contradicts with the assumption
%    %    $\Gammaset  = \emptyset$.
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}\label{R1}
    Let $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$ satisfy the assumption (\ref{assumption_I}).
    If
    \[
    \Gammaset  = \emptyset ,
    \]
     then $\ups_0$ does not satisfy the condition (D) with $(\ups_1, \ups_2, \ups_3)$, for any $\hat{s} > 0$.
\end{prop}
\begin{proof}
    To check the condition (D), we follow similar ideas as before.
    We consider the following two cases, either $({\cap_{j=1}^{3}\gamma_{\ups_j}(\mathbb{R_+})}) \cap J(\ymi, \ypl)$ is empty or not.

    For the first case,
    %it can be shown by the same argument used in Proposition \ref{pp_intersectempty} (1)
    by Proposition \ref{pp_intersectempty},
    we have $(p, \eta) \notin \wfset({\Uthree})$.
    For the second case, let $A =( {\cap_{j=1}^{3}\gamma_{\ups_j}(\mathbb{R_+})}) \cap J(\ymi, \ypl)$.
    By Lemma \ref{lm_finite}, the nonempty set $A$ is finite so we assume $A = \{q_1, \ldots, q_m \}$.
    Since $\gamma_{\ups_0}(\mathbb{R}_-)$ is away from $A$, there exist small open neighborhood $N_k$ of each $q_k \in A$, such that
    $\gamma_{\ups_0}(\mathbb{R}_-) \cap N_k = \emptyset$.

    In the following, we consider the term $\lR_+(w_{(1,1,1)})$ as before.
    Recall $v_l \in I^\mu(\Lambda_l), l=1,2,3$ are Lagrangian distributions away from $p_j$.
    By \cite[Theorem 1.3.6]{Duistermaat2010}, we have
    \[
    \wfset(v_1v_2v_3) \in (\cup_{j=1}^3\Lambda_j) \cup (\cup_{j\neq k \in \{1,2,3\}} \Lambda_j + \Lambda_k) \cup (\Lambda_1 + \Lambda_2 + \Lambda_3),
    \]
    where $\Lambda_j + \Lambda_j$ is defined as before and
    \[\Lambda_1 + \Lambda_2 + \Lambda_3 \coloneqq \{(q, \zeta^{1} + \zeta^{2} + \zeta^{3}): (q, \zj) \in \Lambda_j, j=1,2,3\}.
    \]
    Note that if $(p, \eta)$ is in  $\wfset(\lR_+(w_{1,1,1}))$, then we must have either $(p, \eta) \in \wfset(v_1v_2v_3)$ or there exists $(q, \zeta) \in \wfset(v_1v_2v_3)$ satisfying $(p, \eta)$ is in the null bicharacteristics starting from $({q, \zeta})$, by Lemma \ref{lm_propagation}.
    By the analysis in the proof of Proposition \ref{pp_intersectempty},
    %For the first situation, we must have $y$ contained in $\pi(\Lambda_j)$ for some $j = 1,2,3$.
    %Since $\pi(\Lambda_j)$ tends to $\gamma_{x'_j, \xi'_j}(\mathbb{R}_+)$ as $s_0 \rightarrow 0$, we can always choose $\hat{s}$ small enough such that with $s_0 \in (0, \hat{s})$ one has $y \notin \pi(\Lambda_j)$.
    %For the second situation, first we consider if $(p, \zeta) \in \Lambda_j$, for some $j \in \{1,2,3\}$ and sufficiently small $s_0$.
    %This is impossible, otherwise we have $y \in \gamma_{x'_j, \xi'_j}(\mathbb{R}_+)$.
    %Next, we consider if $(p, \zeta) \in \Lambda_i + \Lambda_j$, for some $i,j \in \{1,2,3\}$ and sufficiently small $s_0$.
    %If so, then $\zeta = \zi + \zj$ with $(p, \zi) \in \Lambda_i$ and $(p, \zj) \in \Lambda_j$.
    %Recall that if a covector $\zeta = \zi + \zj$ is lightlike, then we must have $\zeta$ is propositional to either $\zi$ or $\zj$ by \cite{Kurylev2018}.
    %Then $(p, \zeta)$ is contained either in $\Lambda_i$ or $\Lambda_j$.
    %By the analysis above, this is impossible.
    it suffices for us to consider if  $(q, \zeta) \in \Lambda_1 + \Lambda_2 + \Lambda_3$.
    This happens when we can find some $q = \gamma_{\ups_0}(t_p)$ in $\pi(\Lambda_1 \cap \Lambda_2 \cap\Lambda_3)$.
    Then we apply Lemma \ref{lm_Nk} to $\ups_j$, $j = 1,2,3$.
    Indeed, for sufficiently small $s_0$, the intersection $\pi(\Lambda_1 \cap \Lambda_2 \cap\Lambda_3)$
    is contained in $\cup_{k=1}^m N_k$, where $N_k$ is the small neighborhood of $q_k$ chosen above.
    Since $\gamma_{\ups_o}$ is away from $\cup_{k=1}^m N_k$, there does not exist such $q$.
    %This case is also impossible.
    Thus, we must have $(p,\eta) \notin \wfset(\lR_+(w_{(1,1,1)}))$ and then it is not in  $\wfset(\Uthree)$. To conclude,  the condition (D) does not hold.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lm}[{\cite[Lemma 9.13]{Beem2017}}]\label{lm_twonull}
    If there are two future directed null geodesic segments from $p$ to $q$, then $q$ comes on or after the null cut point of $p$ on each of the two segments.
\end{lm}
\begin{lm}\label{lm_R2_imply}
    Let $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$ and {\blue $\gamma_{\ups_j}$ are not identical} for $j=0,1,2,3$. %satisfy the assumption (\ref{assumption_I}).
    Assume there exists
    $q \in \Gammaset$ such that
    $q = \gamma_{\ups_0}(t_0)$ with $t_0 \in (-\rho(\ups_0^{-}), 0]$ and
    \[
    q = \gamma_{\ups_j}(t_j), \text{ with } t_j \in [0, \rho(\ups_j)), \quad j=1,2,3.
    \]
    where $\ups_0^- \coloneqq (y, -w) \in L^-V$ if we write $\ups_0 = (y, w)$.
    In addition, assume \[
    \dot{\gamma}_{\ups_0}(t_0) \in \text{span}(\dot{\gamma}_{\ups_1}(t_1), \dot{\gamma}_{\ups_2}(t_2), \dot{\gamma}_{\ups_3}(t_3)).
    \]
    Then we have
    \begin{itemize}
        \item[(1)] $q \in \nxxi$ and $y \in \nxxi$, for the definition of $\nxxi$ see (\ref{def_nxxi});
        \item[(2)] in $\nxxi$, the null geodesics $\gamma_{\ups_i}$ and  $\gamma_{\ups_j}$ intersect only at $q$, for any $1 \leq i < j \leq 3$;
        %\item[(3)] there exist $(p_j, w_j) \in \lA(\ups_j)$, where $p_j \neq q$ and are causally independent, see (\ref{assump_xj}), for $j = 1,2,3$;
        \item[(3)] the lightlike vector $\dot{\gamma}_{\ups_1}(t_1), \dot{\gamma}_{\ups_2}(t_2), \dot{\gamma}_{\ups_3}(t_3)$ are linearly independent.
    \end{itemize}
\end{lm}
\begin{proof}
    For (1), with the assumptions above one has $q \in \nxxi$.
    To show $y \in \nxxi$, we prove by contradiction.
    Assume this is not true.
    Then there is $j \in \{1,2,3\}$ such that $y \in J^+(p_j)$, where $p_j = \gamma_{\ups_j}(\rho(\ups_j))$.
    This implies that we can find a causal path $\alpha$ from $p_j$ to $y$.
    Consider the causal path from $q$ to $p_j$ along $\gamma_{\ups_j}$ and then from $p_j$ to $y$ along $\alpha$, which we denote by $\beta$.
    %Note that $\beta$ is not the same with $\gamma_{\ups_0}$, otherwise $\gamma_{\ups_0}$ and $\gamma_{\ups_1}$ are identical.
    If $\beta$ coincide with $\gamma_{\ups_j}$, then we find two null geodesic segments $\gamma_{\ups_j}$ and $\gamma_{\ups_0}$ from $q$ to $y$.
    It contradicts with $t_0 \in (-\rho(\ups_0^{-}), 0]$ by Lemma \ref{lm_twonull}.
    Otherwise, by the short-cut argument in Lemma \ref{lm_shortcut}, we get a contradiction.
    Thus, we must have $q \in \nxxi$.

    For (2), if there is another point $q' \in \nxxi$ such that $q' \in \gamma_{\ups_i}(\mathbb{R}_+) \cap \gamma_{\ups_j}(\mathbb{R}_+)$, then there are two null geodesic segments from $q'$ to $q$ or $q$ to $q'$.
    By Lemma \ref{lm_twonull} we have $q \notin \nxxi$, which contradicts with the assumption.

%    For (3), similarly we prove by contradiction.
%    Assume there exists $p_i, p_j$ such that $p_j \in J^+(p_i)$.
%    Then there is a causal path from $p_i$ to $p_j$ and a null geodesic $\gamma_{\ups_j}$ from $p_j$ to $q$. The same argument in (1) implies $q \notin \nxxi$, which contradicts with the assumption.

    For (3), if this is not true, then without loss of generosity we can assume
    \[
    \dot{\gamma}_{\ups_1}(t_1) \in \text{span}(\dot{\gamma}_{\ups_2}(t_2),\dot{\gamma}_{\ups_3}(t_3))).
    \]
    It follows that
    $\dot{\gamma}_{\ups_1}(t_0) \in \text{span}(\dot{\gamma}_{\ups_2}(t_2), \dot{\gamma}_{\ups_3}(t_3))$.
    {\blue When $\gamma_{\ups_j}$ not identical} for $j=0,1,2,3$, this is impossible, for example,
    by \cite[Lemma 6.21]{feizmohammadi2021inverse}.
\end{proof}
%\begin{corollary}
%    Assume everything above in Lemma \ref{lm_R2_imply}. Then $(\ups_0, \ups_1, \ups_2, \ups_3)$ satisfy the assumption (\ref{assumption_I}).
%\end{corollary}
\begin{prop}\label{pp_R2}
    Let $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$ and {\blue $\gamma_{\ups_j}$ are not identical} for $j=0,1,2,3$.
    Assume there exists
    $q \in \Gammaset$ such that
    $q = \gamma_{\ups_0}(t_0)$ with $t_0 \in (-\rho(\ups_0^{-}), 0]$ and
    \[
    q = \gamma_{\ups_j}(t_j), \text{ with } t_j \in [0, \rho(\ups_j)), \quad j=1,2,3.
    \]
    where $\ups_0^- \coloneqq (y, -w) \in L^-V$ if we write $\ups_0 = (y, w)$.
    In addition, assume \[
    \dot{\gamma}_{\ups_0}(t_0) \in \text{span}(\dot{\gamma}_{\ups_1}(t_1), \dot{\gamma}_{\ups_2}(t_2), \dot{\gamma}_{\ups_3}(t_3)).
    \]
    Then $\ups_0$ satisfies the condition (D) with $(\ups_1, \ups_2, \ups_3)$ and $\hat{s} >0$ small enough.
\end{prop}
%\begin{proof}
%    %    For (1),
%    %    let $s_0, s_1, (\xprimej), f_j$ be as in condition (D).
%    %    When $\capgammathree = \emptyset$, with $s_1$ small enough, one has ${\cap_{j=1}^{3}\gamma_{x'_j, \xi'_j}(\mathbb{R}_+)} = \emptyset$ and $(y, \eta) \notin {\cup_{j=1}^{3}\gamma_{x'_j, \xi'_j}(\mathbb{R_+})}$.
%    %    With $s_0$ small enough, we have $(y, \eta) \notin \cup_{j=1}^{3}\Lambda(x'_j, \xi'_j, s_0)$.
%    %    To simplify the notations, we denote $\gamma_{x'_j, \xi'_j}$ by $\gamma_j$ and $\Lambda(x'_j, \xi'_j, s_0)$ by $\Lambda_j$ below.
%    %    First we consider the case where locally there are exactly two null geodesics
%    %    intersecting at one point.
%    %    Suppose $\gamma_i$ and $\gamma_j$ intersect at a point $p$ with $p \notin \gamma_k$,  where $\{i,j,k\} = \{1,2,3\}$.
%    %    With $s_0$ small enough, suppose $p \notin K_k$.
%    %    %With $s_0$ small enough we can assume $\cap_{j=1}^3 K_j = \emptyset$.
%    %    Note that we do not assume $p \in \nxxi$.
%    %    In other words, we could have cut points before $p$ along $\gamma_i$ or $\gamma_j$.
%    %    In general $v_l \in \Ical^\mu(\Lambda_l)$ are Lagrangian distributions associated with the Lagrangian submanifold $\Lambda_l$.
%    %    %may not be a conormal distribution supported in $K_l$, $l = 1,2,3$.
%    %    We consider the wave front set of a model term $Q_g(v_i v_j v_k)$ using the H\"{o}rmander-Sato Lemma and the propagation of singularities.
%    %    Indeed, since $v_k$ is smooth near $p$, the wave front set of $v_i v_j v_k$ at $p$ is in the span of $\Lambda_i$ and $\Lambda_j$.
%    %    Let $(p, \zeta^{(i)}) \in \Lambda_i$ and $(p, \zeta^{(j)}) \in \Lambda_j$.
%    %    If a covector $\zeta = \zi + \zj$ is lightlike, then we must have $\zeta$ is propositional to either $\zi$ or $\zj$ by \cite{Kurylev2018}.
%    %    Thus, there are no new singularities produced other than $\cup_{j=1}^3 \Lambda_j$, if we apply $Q_g$ to $v_i v_j v_k$.
%    %    For the terms in form of $Q_g(\cjv_iv_jv_k)$ or $Q_g(\lge A_1, \diff v_i \rge_g \cjv_j v_k)$, %, or $\lge A_1, \diff \cjv_i \rge_g v_j v_k$,
%    %    we only need to notice that $\wfset(\cjv_i)$ or $\wfset(\lge A_1, \diff v_i\rge)$ is contained in  $\Lambda_i$.
%    %    In the case that none of three geodesics intersect with each other, we have $\wfset(v_i v_j v_k) \subset \cup_{j=1}^3 \Lambda_j$ and it follows that
%    %    $\wfset(Q_g(v_i v_j v_k)) \subset \cup_{j=1}^3 \Lambda_j$.
%    %    In both cases,  we can conclude that $(y, \eta) \notin \wfset(Q_g(v_i v_j v_k))$, since
%    %    %with the assumption $y \notin \uniongammathree$, if $s_0$ is sufficiently small.
%    %    Thus, one has $(y, \eta) \notin \wfset(\mathcal{U}^{(3)})$, which implies the condition (D) is not satisfied.
%    %    The second statement
%    %, when $A_1$, $\divg(A_1)$, or $h_1$ is nonvanishing at $q$.
%    %    Note that the assumptions above imply that $q \in \nxxi$ and $y \in \nxxi$,
%    %    %Note that $(y, \eta) \in \mathcal{C}^{\text{reg}}(q, \zeta, t_y)$ implies $y \in \nxxi$,
%    %    otherwise we can use the shortcut arguments to show $t_y > \rho(q, \zeta)$.
%    %    It follows that $q$ is the only intersection point of $\gamma_{\ups_j}(\mathbb{R}_+)$ in $\nxxi$ for $j=1,2,3$, otherwise there would be cut points.
%    %
%    %    Then this statement comes from
%    Note that
%    By Lemma \ref{lm_R2_imply}, we can apply Proposition \ref{pp_three}, when the assumption (\ref{assumption_Ah}) holds.
%    %    suppose we choose $f_1, f_2, f_3$ as in Section \ref{subsec_A1h1}
%    %    such that
%    %    \begin{itemize}
%        %        \item[(1)] $\sigma^{(p)}(v_j) =  0$ near $(q, \zj)$ and
%        %        $ \sigma^{(p)}(v_j)\neq 0$ near $(q, -\zj)$, for $j = 1$,
%        %        \item[(2)] $\sigma^{(p)}(v_j) \neq  0$ near $(q, \zj)$ and
%        %        $ \sigma^{(p)}(v_j)= 0$ near $(q, -\zj)$, for $j = 2,3$.
%        %    \end{itemize}
%    Indeed, if $q \in  \mathcal{O}(A_1)$,  by (\ref{def_OA1}) either $A_1(q) \neq 0$ or $A_1 = 0$ near $q$.
%    When $A_1$ vanishes near $q$, we must have $h_1(q) \neq 0$ with the assumption (\ref{assumption_Ah}), and therefore
%    \[
%    \mathcal{U}^{(3)} \in \mathcal{I}^{3\mu + \frac{1}{2}} ( \Lambda_{123}^g),
%    \]
%    away from $(\cup_{j=1}^3 \Lambda_j) \cup \Lambda_{123}$.
%    For $j=1,2,3$, we can choose $(x_j',\xi_j') = (x_j, \xi_j)$ and $f_j \in  I^{\mu}(\Sigma(x_j',\xi_j',s_0))$ as in Section \ref{subsec_A1h1}.
%    In this case, the principal symbol
%    \[\begin{split}
%        \sigma^{(p)}(\mathcal{U}^{(3)})(y, \eta) =- 2(2\pi)^{-2} \sigma^{(p)}(Q_g)(y, \eta,q, \zeta)
%        h_{1}(q)
%        \overline{\sigma_1(q, -\zeta^{(1)})} \sigma_2(q, \zeta^{(2)})\sigma_3(q, \zeta^{(3)}),
%    \end{split}\]
%    is nonvanishing and it follows that $(y, \eta) \in \wfset(\mathcal{U}^{(3)})$.
%    When $A_1 \neq 0$ at $q$, we have
%    \[
%    \mathcal{U}^{(3)} \in \mathcal{I}^{3\mu + \frac{3}{2}} ( \Lambda_{123}^g),
%    \]
%    away from $(\cup_{j=1}^3 \Lambda_j) \cup \Lambda_{123}$.
%    By (\ref{eq_U3special}), its principal symbol is given by
%    \[\begin{split}
%        \sigma^{(p)}(\mathcal{U}^{(3)})(y, \eta)
%        =
%        (2\pi)^{-2} \sigma^{(p)}(Q_g)(y, \eta,q, \zeta)
%        \lge A_1, 3\zeta -\zeta^{(1)} \rge_g
%        \overline{\sigma_1(z, -\zeta^{(1)})} \sigma_2(z, \zeta^{(2)})\sigma_3(z, \zeta^{(3)}).
%    \end{split}\]
%    Note that the quantity $\lge A_1, 3\zeta -\zeta^{(1)} \rge_g$ may vanish at $q$ with $(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)})$ %$(\zj)_{j=1}^3$,
%    but we can always fix $\zeta$ and perturb $\zeta^{(1)}$ slightly to get a lightlike covector $\theta^{(1)}$ such that
%    $\lge A_1, 3\zeta -\theta^{(1)} \rge_g \neq 0$.
%    Indeed, by the same idea as in the proof of Lemma \ref{lm_perturb_y}, we can find
%    $\varsigma >0$, such that for any $\theta \in N^+(\zeta^{(1)}, \varsigma)$
%    there exists a covector
%    $(x, \xi) \in L^{*,+} V$ with $(q, \theta) = \mathcal{C}^{\text{reg}}(x, \xi, t_q)$ for some $t_q >0$.
%    Let $\theta^{(1)} = \theta$.
%    Then by Corollary \ref{cor_3null}, one can find $\theta^{(2)}, \theta^{(3)} \in L^+V$, as the perturbation of $\zeta^{(2)}, \zeta^{(3)}$ such that $\theta^{(j)}$ are linearly independent and $\zeta$ is in their span.
%    %For more details, see Corollary \ref{cor_3null}.
%    Let $b_j=(\theta^{(j)})^\#$ and we define  $(x_j',\xi_j')$ by reversing the flow from $(q,b_j)$, i.e. define
%    $x_j' = \gamma_{q, b_j}(-t_j)$ and $\xi_j' = \dot{\gamma}_{q, b_j}(-t_j)$.
%    With small enough perturbation, we can assume $q \in {{\mathcal{N}(\vec{x}', \vec{\xi}')}}$.
%    Then one can construct $f_j \in I^{\mu}(\Sigma(x_j',\xi_j',s_0))$ as in Section \ref{subsec_A1h1} and it follows that $(y, \eta) \in \wfset(\mathcal{U}^{(3)})$.
%    %   For (3), the source-to-solution map determines $\mathcal{U}^{(3)} = \partial_{\ep_1}\partial_{\ep_2}\partial_{\ep_3} L(f)|_{\ep_1 = \ep_2 = \ep_3  = 0}$ and therefore it determines the condition (D).
%    %%
%    %%   \begin{lm}\label{lm_3null2}
%        %%   Let $q \in I(p^-,p^+)$.
%        %%   Suppose
%        %%   \end{lm}
%    %%
%    %%   but with Claim \ref{cl_generic}
%    %%   it is nonvanishing on any open subset of $\mathcal{Y}$.
%    %%   we can always make arbitrarily small perturbation to find linearly independent lightlike covectors $(\theta^{(j)})_{j=1}^3$ such that $\lge A_1, 3\theta -\theta^{(1)} \rge_g \neq 0$, where $\theta = \sum_{j=1}^3 \theta^{(j)}$.
%    %%   In addition, to detect the singularities at $(y, \eta)$, we need that $\zeta$ is in the span of $(\theta^{(j)})_{j=1}^3$, i.e., $\det(\zeta,  \theta^{(1)},  \theta^{(2)}, \theta^{(3)}) = 0$.
%    %%
%    %%   Let $b_j=(\theta^{(j)})^\#$. Then we define  $(x_j',\xi_j')$ by reversing the flow from $(q,b_j)$, i.e. define
%    %%   $x_j = \gamma_{q, b_j}(-t_j)$ and $\xi_j' = \dot{\gamma}_{q, b_j}(-t_j)$.
%    %%
%\end{proof}

Now we define the following relation
\[\begin{split}
    R_L &= \{(\ups_0, \ups_1, \ups_2, \ups_3)
    \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3:
    \text{ they are corresponding to distinct null geodesics}\\
    &\quad \quad \quad \quad \quad \quad\quad \quad \quad\quad \quad \quad\text{and there exists } \hat{s}>0
       \text{ such that (D) is} \text{ valid for }
    \ups_0 \text{ with } (\ups_1, \ups_2, \ups_3)
    \}.
\end{split}\]
We verify that $R_L$ is a three-to-one scattering relation by the following proposition.
\begin{prop}\label{pp_RL}
    The relation $R_L$ defined above is a three-to-one scattering relation for all points $q \in M$.
    Moreover,
    using the nonlinear radiation field and the extended metric, one can determine whether $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$ is in the relation $R_L$.
\end{prop}
\begin{proof}
    Let $(\ups_0, \ups_1, \ups_2, \ups_3) \in L^{+}_{S_+}M \times (L^{+}_{S_-}M)^3$.
    Proposition \ref{R1} shows the first condition (R1) in Definition (\ref{def_3to1}) is satisfied
    and Proposition \ref{pp_R2} shows the second condition (R2) is satisfied.

    Note that the condition (D) is determined by the nonlinear radiation field.
    %and $\lA(\ups)$ is uniquely determined by the extended metric.
    Additionally, one can check if the assumption (\ref{assumption_I}) holds for $(\ups_0, \ups_1, \ups_2, \ups_3)$ using the nonlinear radiation field.
    It follows that $R_L$ is determined by them.
\end{proof}
%Thus, by \cite[Thoerem 1.3]{feizmohammadi2021inverse}, the conformal class of the Lorentzian metric at points in $I(\imi, \ipl)$ is uniquely determined up to conformal factors and diffeomorphisms.
%Since $\mathcal{O}(A_1)$ is dense in $I(p^-, p^+)$ and the metric tensor is smooth, it determines the conformal class of the Lorentzian metric up to diffeomorphisms at all points in $I(p^-, p^+)$.
%%By \cite{Feizmohammadi2020a}, first we define a conical piece
%%\[
%%CP(v_1, v_2) = \{v_0: \text{ there is } v_3 \in L^+ U \text{ such that } (v_0, v_1, v_2, v_3)\in R_L\}.
%%\]
%%Then let
%%\[\begin{split}
%%\mathcal{C}(v_1, v_2) & = \{C \subset L^+U: C \subset CP(v_1, \tilde{v}) \cap CP(v_2, \tilde{w}) \text{ for some }\\
%%&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \tilde{v}, \tilde{w} \text{ satisfying } \gamma_{v_1} \neq \gamma_{\tilde{v}}, \gamma_{v_2} \neq \gamma_{\tilde{w}} \}.
%%\end{split}\]
%%We define
%%\[
%%P(v_1, v_2) = \{\pi(u): u \in \cup_{C \in \mathcal{C}(v_1, v_2)} C\}
%%\]
%%and
%%\[
%%E_U(v_1, v_2) = \bigcap_{a \in \mathcal{A}} \textbf{e}_a(\text{cl}(P(v_1, v_2)).
%%\]
%%\begin{prop}
%%Let $v_j = (x_j, \xi_j) \in L^+ U$ and suppose that there is $q  = \gamma_{x_j, \xi_j} (t_j)$ satisfying $t_j \in (0, \rho(x_j, \xi_j))$ for $j=1,2$.
%%Then
%%
%%
%%
%%\end{prop}
%%
%%\begin{prop}[{Analog of \cite[Theorem 4.5]{Kurylev2018}}]
%%Assume that for all $ (\vec{x}, \vec{\xi}) = ((x_j, \xi_j))_{j=1}^3 \in (L^+U)^3$, such that () is valid.
%%We write $v_j = (x_j, \xi_j)$ and suppose there are sets $S_0(v_1, v_2)$ satisfy the following properties:
%%\begin{itemize}
%%    \item[(P1)] If there is $q \in J^-(p^+)$ such that $q  = \gamma_{x_j, \xi_j}(t_j)$ with $t_j \in (0, \rho(x_j, \xi_j))$ for $j = 1, 2, 3$, then $S_0(v_1, v_2) = \mathcal{E}_U(q)$.
%%    \item[(P2)] If there are no such $q \in J^-(p^+)$, then $S_0(v_1, v_2) \subset M \setminus \mathcal{N}$.
%%\end{itemize}
%%\end{prop}
%The analysis above indicates the following theorem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{thm}\label{thm_Lmetric}
%    Let $G_k$ be two globally hyperbolic Lorentzian metrics on $X = \mathbb{R} \times \mR$ for $k=1,2$, satisfying assumptions H1-H3 and NL.1-NL.2.
%    Let $\mcn_k$ be the corresponding nonlinear Friedlander radiation field defined in (\ref{def_mcn}) for the nonlinear equation
%    \[
%    \sq_{G_{k}} u + u^3 = 0, \quad \text{ for } k = 1,2.
%    \]
%    If $\mcn_1 = \mcn_2$, then there is a conformal diffeomorphism $\Psi: (X, G_1) \rightarrow (X, G_2)$.
%\end{thm}






